Handover Protocol Learning for LEO Satellite Networks: Access Delay and Collision Minimization

This study presents a novel deep reinforcement learning (DRL)-based handover (HO) protocol, called DHO, specifically designed to address the persistent challenge of long propagation delays in low-Earth orbit (LEO) satellite networks' HO procedures. DHO skips the Measurement Report (MR) in the HO procedure by leveraging its predictive capabilities after being trained with a pre-determined LEO satellite orbital pattern. This simplification eliminates the propagation delay incurred during the MR phase, while still providing effective HO decisions. The proposed DHO outperforms the legacy HO protocol across diverse network conditions in terms of access delay, collision rate, and handover success rate, demonstrating the practical applicability of DHO in real-world networks. Furthermore, the study examines the trade-off between access delay and collision rate and also evaluates the training performance and convergence of DHO using various DRL algorithms.

==> Section/Repo/SEC1_CY.tex <==
\subsection{\tblue{Related Works}}
% \tblue{
% "Access scheme + DRL"
1) Communication and networking에 DRL을 적용한 work에 대한 survey 논문~\cite{8714026}

2) A primary-prioritized recurrent deep reinforcement learning algorithm for dynamic spectrum access based on cognitive radio (CR) technology is proposed.~\cite{9557877}

3) This paper investigates the communication strategies of a distributive DSA network under the presence of spectrum sensing errors. + Apply DRL for SUs(secondary users) to learn “appropriate” spectrum access strategies in a distributed fashion assuming NO knowledge of the underlying system statistics.~\cite{8474348}

4) This paper investigates deep reinforcement learning (DRL) based on a Recurrent Neural Network (RNN) for Dynamic Spectrum Access (DSA) under partial observations, referred to as a Deep Recurrent Q-Network (DRQN).~\cite{9089307}

% "LEO SAT+DRL"
5) 데이터 처리량, 대역폭 및 전력과 관련된 여러 목표를 달성하기 위해 국제우주정거장(ISS) 기반 테스트베드에서 지상국까지의 space link를 구성함. 이 때 머신 러닝을 사용하여 최적의 궤도를 강화 학습을 기반으로 산출하기 위한 테스트 수행~\cite{8713802}.

6) Satellite Internet of Things(SIoT)에서 LEO 위성에 적합하면서 에너지 효율적인 채널 할당을 위한 강화 학습 기반 접근 방식 제안~\cite{9047860} 

7) 이주형 박사님 2020 GLOBECOM 논문~\cite{P4C_JH}

% "HO + LEO SAT"
8) LEO satellite communication networks에서 Graph 기반(Satellite과 User 관계)의 핸드오버 scheme 제시~\cite{7470617}

9) Satellite handover strategy based on the \textbf{potential game} for mobile terminals in a LEO satellite communication network.~\cite{8836603}

10) Proposes a handover strategy for the links between satellites and gateway stations based on w\textbf{eighted bipartite graph} in LEO satellite networks using Kuhn-Munkres (KM) algorithm.~\cite{9068245}
% }


==> Section/Repo/SEC2_CY.tex <==
HO (HO) is the process of transferring an ongoing data session (or call) from one cell in a cellular network to another without interruption. 

Generally, the process of HO can be divided into three main stages:
\textit{i)} detection of the need for HO and decision on the target cell for HO,
\textit{ii)} execution of the HO,
and \textit{iii)} completion of the HO.
It is worth noting that the HO process is done by the BS and UE working together. Thus, the HO success rate depends on several aspects of each entities, e.g., the network conditions, the mobile device's capabilities, and the design of the cellular network.

\subsection{Overview of HO Process} \label{sec:HO_overview}
In a Long Term Evolution (LTE) communication network, a UE participating in LTE communication refers to a user's communication equipment and all equipment capable of accessing mobile communication. The UE attempts to connect to the base station to use a communication service. At this time, the base station to which the UE directly requests connection is called an eNodeB (gNB). The gNB is a device that wirelessly connects to the UE, but the possible range of accepting UE's connection is limited due to the physical limitations of the gNB device. However, the wireless connection between the UE and the currently connected serving gNB(S-gNB) is disconnected when the UE moves out of the range covered by the corresponding S-gNB. Therefore, it is necessary to disconnect the previously connected S-gNB and establish a new connection with a neighboring neighbor gNB (N-gNB) covering the range to which the UE has moved. In particular, LTE HO in the 3rd generation partnership project (3GPP)~\cite{karabulut2019analysis} occurs most often when the UE disconnects from the S-gNB before establishing a new connection with the T-gNB. Consequently, the gNB must perform mobility management to consider the flexible change of UE's position and radio source management including allocating frequencies to UEs. The general HO process based on 3GPP is composed of three steps; \textit{i)} Preparation, \textit{ii)} Execution, and \textit{iii)} Completion~\cite{8959359}. We will describe the three aforementioned air-interface signalling processes in detail with the sequence diagram shown in Fig.~\ref{fig:existing HO process}.
% Long Term Evolution (LTE) 통신망에서 LTE 통신에 참여하는 UE는 사용자가 사용하는 통신 장비로, 이동통신에 접속 가능한 모든 장비를 칭한다. UE는 통신 서비스를 사용하기 위해서 기지국과의 연결을 시도하게 되는데, 이 때 UE가 직접적으로 연결을 요청하는 기지국을 eNodeB (gNB)라고 한다. gNB는 무선(radio)으로 UE와 연결하는 장비인데, gNB 장비의 물리적 한계로 인해 UE의 연결을 수락할 수 있는 범위가 제한되어 있다. 그런데, UE의 이동으로 인해 현재 연결된 serving gNB (S-gNB)가 커버하는 범위를 벗어나게 되면 해당 UE의 무선 통신 연결이 끊어지게 되는 상황이 발생한다.따라서 기존에 연결된 S-gNB와의 연결을 끊고, 해당 범위를 커버하는 이웃한 neighbor gNB (N-gNB)와 새로운 연결을 설정해야 한다. 특히, 3rd generation partnership project (3GPP)~\cite{karabulut2019analysis} 에서 LTE의 핸드오버는 위와 같이 UE가 T-gNB와 새로운 연결을 설정하기 이전에 S-gNB와의 연결을 끊을 때 가장 많이 발생한다. 이와 같이 gNB는 사용자 이동에 의해 접속 가능한 gNB가 유동적으로 변경되는 것을 고려하기 위한 이동성 관리 (mobility management)와 더불어서, UE에 주파수를 할당하는 것을 비롯한 무선 자원 관리 (radio source management)를 수행한다. 일반적으로 3GPP를 기준으로, 핸드오버의 과정은 다음과 같이 크게 3가지 단계로 구성된다; (i) Preparation, (ii) Execution, and (iii) Completion~\cite{8959359}. 다음으로 이 3가지 프로세스에 대해서 Fig.~\ref{fig:existing HO process}의 구조를 가지고 자세히 설명한다.

\begin{table*}
  \centering
  \resizebox{1\linewidth}{!}{\begin{minipage}[t]{1\textwidth}
  \centering
  \caption{The entering condition of HO events.}
  \renewcommand{\arraystretch}{1.0}
  \label{tab:A1_5}
  \centering
  \input{Table/Table_HOevent.tex}
  \centering
  \end{minipage}}
\end{table*} 

\begin{enumerate}
    \item \textsf{Preparation phase} : 
    Generally, HO occurrence conditions are measured on the basis of the downlink (DL) reference signal received power (RSRP). Therefore, the UE measures signals of the S-gNB and N-gNBs to periodically evaluate whether the measured signals satisfy the conditions for a HO event. In LTE, five HO event entry conditions can be considered as shown in Table~\ref{tab:A1_5}; the A3 event is the most widely used among them~\cite{8959359}. This paper names the N-gNB designated as the HO receiver target gNB (T-gNB) during the HO process. In order to know the HO event occurrence condition based on RSRP, the HO margin (HOM), which is the minimum received power or quality between S-gNB and N-gNB as a candidate for T-gNB, is generally used as a standard. To differentiate the HO event occurrence condition based on RSRP, the S-gNB generally used HOM (HO Margin) as a standard where HOM is the minimum received power or quality between the S-gNB and N-gNB that is a T-gNB candidate. Next, time-to-trigger (TTT) measured in seconds is the minimum time that the HOM condition must be satisfied for a HO event to occur. In other words, the HOM of the N-gNB corresponding to the T-gNB candidate must be better than the S-gNB for at least TTT seconds for occurring HO~\cite{alonso2010self}. If the HO event occurrence condition is satisfied within the TTT period, the UE sends a \texttt{Measurement Report} (\texttt{MR}) to the S-gNB. The measurement report comprises several channel quality-related parameters, \textit{i.e.}, the RSRP, the reference signal received quality (RSRQ), and the received signal strength indicator (RSSI)~\cite{9813555, yajnanarayana20205g}. Before starting the HO process, the S-gNB determines which T-gNB to perform HO to based on \texttt{MR} sent by the UE. After that, the S-gNB sends \texttt{HO Request} to the T-gNB to discriminate whether the T-gNB can perform HO. If the T-gNB that received the request accepts the HO request, it returns an \texttt{HO Request Acknowledgment} (\texttt{ACK}) to the S-gNB. Here, \texttt{ACK} is a reply sent when a packet is successfully transmitted to the communication target. After receiving the \texttt{HO Request ACK} back, the S-gNB sends a \texttt{HO Command} to the UE to move on to the \textsf{Execution phase} where the HO process is carried out in earnest.
    % 일반적으로 downlink (DL) reference signal received power (RSRP)를 기반으로 핸드오버의 발생 조건을 측정한다. 따라서, UE는 S-gNB와 N-gNB들의 신호를 측정하고, 측정된 신호가 핸드오버 이벤트가 발생할 조건을 충족하는지 평가한다. 이 때 LTE에서는 Tab.~\ref{tab:A1_5}와 같이 5가지의 핸드오버 이벤트 진입 조건을 고려할 수 있으며, 그 중에서 A3 이벤트가 가장 널리 사용되고 있다~\cite{8959359}. 이 논문에서는 핸드오버 프로세스가 진행되는 동안에 S-gNB와 핸드오버 수신자로 지정된 N-gNB를 \textit{target gNB}(T-gNB)라고 칭한다. RSRP를 기반으로 핸드오버 이벤트 발생 조건을 알기 위해서는 일반적으로 데시벨 단위의 HO margin (HOM)를 기준으로 삼으며, HOM은 T-gNB의 후보에 해당하는 N-gNB와 S-gNB 간의 최소 수신 전력 또는 품질이다. 다음으로, 초 단위로 측정되는 time-to-trigger (TTT)는 핸드오버 이벤트가 발생하기 위해 HOM 조건이 충족되어야 하는 최소 시간이다. 다시 말해서, 핸드오버 발생을 위한 조건은 T-gNB의 후보에 해당하는 N-gNB의 HOM이 적어도 TTT 초 동안 S-gNB보다 좋아야 하며~\cite{alonso2010self}, 만약 핸드오버 이벤트 발생 조건이 TTT 기간 내에 충족된다면 UE는 \texttt{Measuremet Report (MR)}를 S-gNB에게 보낸다. S-gNB는 핸드오버 프로세스를 시작하기 전에, UE가 보낸 \texttt{MR}을 기반으로 어떤 T-gNB로 핸드오버를 수행할지 결정한다. 이후, T-gNB가 핸드오버를 진행할 수 있는 상태인지 알기 위해서 \texttt{HO Request}를 T-gNB에게 보내고 해당 T-gNB가 핸드오버 요청을 받아들인다면, 다시 S-gNB에게 \texttt{HO Request ACK}를 돌려보낸다. 
    % 여기서 ACK란, Acknowledgment의 약자로 통신대상에게 성공적으로 패킷이 전송되었는지를 알기 위한 답신이다. \texttt{HO Request ACK}를 돌려 받은 S-gNB는 UE에게 \texttt{HO Command}를 보내어 본격적인 핸드오버 프로세스를 진행하는 \textsf{Execution phase}로 넘어간다.
   
    \item \textsf{Execution phase} : 
    When communicating between a UE and a base station, we can divide a communication link into two types according to directionality; Uplink (UL) and DL. UL means a transmission path from a terminal to a base station, and DL means the opposite. Sequence numbers (SNs) are used to distinguish these two types of communication links. In the \textsf{Execution phase}, the S-gNB transmits the UE's DL data and \texttt{SN Status Transfer} including a packet data convergence protocol (PDCP) sequence number to the T-gNB~\cite{alexandris2016analyzing}. PDCP assigns numbers to data blocks in order through sequence numbering so that the receiving side can know the order and duplication of packets that have arrived. Upon receiving the \texttt{HO command}, the UE disconnects from the S-gNB and executes a random access channel (RACH) based connection process with the T-gNB~\cite{hasan2013random, 7878690} as shown in Fig.~\ref{fig:existing HO process}. We describe the overall process of RACH as follows: \textit{i)} UEs attempting to access one T-gNB indicate the starting point of data transmission so that the T-gNB estimates the delay with the UE and then randomly selects a preamble enabling synchronization. At this time, if two or more UEs select the same preamble at the same time, a collision occurs. The T-gNB monitors whether a specific preamble is activated to detect such a collision~\cite{6477838}. \textit{ii)} The T-gNB transmits a \texttt{Random Access} (\texttt{RA}) \texttt{Response} corresponding to each activated preamble. It allocates resources to the UE by delivering physical parameters such as timing advance (TA) that has activated the preamble. When the T-gNB sends a signal to UEs separated by different distances, it arrives at the UE at different times, and signal interference occurs. Therefore, a physical parameter such as TA is required to solve the timing problem during synchronization. \textit{iii)} Upon receiving the RA response for preamble activation, each UE sends a \texttt{Radio Resource Control} (\texttt{RRC}) \texttt{Connection Request} to the T-gNB to receive resources for subsequent data transmission. If two or more UEs activate the preamble, all corresponding UEs transmit an RRC connection request using the same resource. The T-gNB can detect the preamble activation collision. \textit{iv)} Finally, the T-gNB schedules the colliding UEs to wait for a random time and then try again through a predefined RA protocol, such as ALOHA, slotted ALOHA, CSMA, and CSMA-CD. When the UE can access the T-gNB as a result of a successful HO, the UE sends a \texttt{HO Confirm} message to the T-gNB to prompt it to send the DL data to the UE~\cite{7462492}.
    % UE와 기지국간에 통신을 할 때 방향성에 따라 두가지로 구분할 수 있다; Uplink (UL), Downlink (DL). UL은 단말에서 기지국으로의 전송 경로를 의미하고, DL은 반대로 기지국에서 단말로의 전송 경로를 의미한다. 이러한 DL 및 UL를 구분하기 위해서 sequence number (SN)를 사용한다.  \textsf{Execution phase}에서는 이를 나타내기 위해 S-gNB는 T-gNB에게 packet data convergence protocol (PDCP) sequence number가 포함되어 있는 \texttt{SN Status Transfer} 메시지를 전송하고, UE의 DL 데이터를 T-gNB로 전달한다~\cite{alexandris2016analyzing}. PDCP는 Sequence numbering을 통해 데이터 블록에 순서대로 번호를 붙여서 수신측에서 도착한 packet의 순서와 중복을 알 수 있게 하며, UL의 경우 첫 번째로 누락된 data unti이 포함되고 DL의 경우 다음 SN이 할당된다. \texttt{HO Command}를 전달받은 UE는 S-gNB와의 연결을 해제하고, Fig.~\ref{fig:existing HO process}과 같은 T-gNB와의 random access channel (RACH) 기반의 연결 과정을 실행한다~\cite{hasan2013random, 7878690}. (i) 하나의 T-gNB (BS)에 접근을 시도하는 각각의 UE는 데이터 전송의 시작 지점을 나타내어 T-gNB가 UE와 자신과의 delay를 추정하도록 함으로써 동기화를 가능하게 하는 preamble을 무작위로 선택한다. 이 때 만약 두 개 이상의 UE가 동시에 동일한 preamble을 선택하면 충돌이 발생하게 되는데, T-gNB는 이러한 충돌을 감지하기 위해서 특정 preamble이 활성화되어 있는지 여부를 감시한다~\cite{6477838}. (ii) T-gNB는 각각 활성화된 preamble에 대응하는 random access (RA) response를 전송하여 preamble을 활성화한 UE에게 timing advance (TA)와 같은 물리적인 parameter를 전달하며 resource를 할당한다. T-gNB가 서로 다른 거리만큼 떨어져 있는 UE들에게 신호를 보내면 서로 다른 시간에 UE에게 도착하여 signal interference가 발생하기 때문에 동기화 시 타이밍 문제를 해결하기 위해서는 TA와 같은 물리적인 parameter가 필요하다. (iii) Preamble 활성화에 대한 RA response를 수신한 각 UE는 후속 데이터 전송을 위한 자원을 요청하기 위해 T-gNB에게 radio resource control (RRC) 연결 요청을 한다. 만약 둘 이상의 UE가 preamble을 활성화한 경우, 해당하는 모든 UE들은 동일한 resource를 사용하여 RRC 연결 요청을 전송하고, T-gNB가 이 충돌을 감지한다.(iv) 마지막으로 T-gNB는 (ALOHA, slotted ALOHA, CSMA, CSMA-CD와 같은) 미리 정의된 RA 프로토콜을 통해 충돌한 UE들이 임의의 시간 동안 대기한 후 다시 접근 시도를 하도록 scheduling 한다. 성공적으로 핸드오버가 수행되어 UE가 T-gNB에게 접근할 수 있게 되면, UE는 T-gNB에게 \texttt{HO Confirm} 메시지를 전달하여 T-gNB가 UE의 DL 데이터를 UE에게 보내도록 prompt한다~\cite{7462492}.
    
    \item \textsf{Completion phase} : 
    When the HO connection between the UE and the T-gNB is completed, the core network entities request to switch the path of the DL packet from the S-gNB to the T-gNB. In the process of switching to a new path, the T-gNB can receive an end marker from the previous path~\cite{alexandris2016analyzing}. When the path-switching process is completed, the T-gNB completes the HO by transmitting \texttt{HO Complete} to release the resources allocated by the UE in context with the S-gNB and the previously established bearer. The bearer, a logical tunnel created between the UE and the gNB, provides a service so that information can be transferred between interfaces in real-time without changing the contents.
    % UE와 T-gNB 간의 핸드오버 연결이 완료되면, Core network entity들이 DL 패킷의 경로를 S-gNB로부터 T-gNB로 switch하도록 요청한다. 새로운 path로 swithing하는 과정에서 T-gNB는 이전의 path로부터 end-marker를 받을 수 있다~\cite{alexandris2016analyzing}. 해당 path switching 과정이 완료되면 T-gNB는 UE가 S-gNB와의 context에서 할당받은 resource들을 release 하기 위해 \texttt{HO Complete}를 전송하여, 기존에 establish된 bearer를 realease하며 핸드오버가 마무리된다. 이 때 bearer란, UE와 gNB 간 생성되는 논리적인 터널로, 인터페이스 상호 간에 정보를 실시간으로 내용의 변경 없이 전달할 수 있도록 서비스를 제공한다.
\end{enumerate}

\begin{figure}
    \centering
    \includegraphics[width=.9\linewidth]{Figure/Fig_HO_Conventional.png}
    \caption{The sequence diagram of existing 3GPP 5G HO schemes.}
    \label{fig:existing HO process}
\end{figure}
When the conditions for HO are met, the signal quality or RSRP of the S-gNB is not good, and the interference of the N-gNBs is severe. Thus, HO may fail due to transmission/reception failure of HO-related messages or occurrence of radio link failure (RLF) by high interference of N-gNBs. In other words, we can say that \textsf{Preparation phase} is the most vulnerable part of the HO process~\cite{hesnet}.
% 핸드오버가 발생하는 조건 자체가 S-gNB의 signal quality 또는 RSRP가 좋지 않거나 N-gNB들의 간섭이 심한 상황이기 때문에 \texttt{MR}과 \texttt{HCMD}와 같은 핸드오버 수행 메시지의 송수신이 실패하거나, 핸드오버 과정 중 높은 간섭이나 UE의 이동성으로 인한 radio link failure (RLF)가 발생하게 되어 핸드오버의 수행이 실패할 수도 있다~\cite{puttonen2010radio}. 즉, \textsf{Preparation phase}가 핸드오버 진행에 있어서 가장 취약한 부분이라고 말할 수 있다~\cite{hesnet}.



==> Section/Repo/SEC3_CY.tex <==
For NTN, in particular, for LEO SAT networks, HO  is considered to be a more challenging procedure than in terrestrial cellular networks for several reasons:
\begin{enumerate}
    \item Long propagation delay: The signal from the mobile device to the satellite and back to the ground station takes a significant amount of time to travel, which can lead to a delay in the handover process.
    \item Interference: The interference caused by other satellites and other sources, such as atmospheric effects, can cause problems in the handover process, making it less reliable.
    \item Large geographical coverage area: The coverage area of a satellite is much larger than that of a terrestrial cell, which can make it more difficult to identify the best target cell for handover.
    \item Limited resources: The limited resources available on a satellite can make it harder to support handover, especially when multiple handovers are required at the same time.
\end{enumerate}
Due to these challenges, handover in satellite communication is considered to be less efficient and less reliable than in terrestrial cellular networks. As a result, techniques such as beam switching and frequency reuse are often used to mitigate the challenges associated with handover in satellite communication.

\subsection{Challenge: Outdated, Power-Consuming, and Unreliable Measurement Report}

\begin{figure*}[t!]
    \centering
    \subfloat[Propagation Delay.]{
    \includegraphics[width=0.333\linewidth]{Figure/Propagation_Delay.eps}
    \label{fig:Propagation_delay}
    }
    \subfloat[Signal--to--Noise Ratio.]{
    \includegraphics[width=0.333\linewidth]{Figure/SNR.eps}
    \label{fig:SNR}
    }
    \subfloat[Bit Error Ratio.]{
    \includegraphics[width=0.333\linewidth]{Figure/BER.eps}
    \label{fig:BER}
    }
    \caption{Multifaced calculations according to the distance between Tx and Rx in the ground-to-satellite uplink signal.}
\end{figure*}

However, there is a limit to using the existing handover method described above as it is in a LEO satellite network. First,the physical distance from the UE on the ground is very long since the LEO satellites provide network services at an altitude of 500--2000 km~\cite{9356529}. Therefore, there is a problem in that a long propagation delay is consumed in transmitting exchanged packets when handover occurs. We can calculate the propagation delay when two terminals exchange a packet as follows:
% 그러나 앞서 설명한 기존 핸드오버 방식을 저궤도 위성 네트워크(LEO Satellite)에서 그대로 사용하기에는 한계가 존재한다. 먼저, 저궤도 위성 네트워크는 500--2000km의 고도~\cite{9356529}에서 네트워크 서비스를 제공하기 때문에 지상의 UE와 물리적인 거리가 매우 길다. 따라서 이러한 물리적인 한계로 인해, 핸드오버 발생 시 주고받는 패킷이 전달되는 데에 긴 propagation delay가 소모된다는 문제를 가지고 있다. 두 단말 간에 패킷을 전달할 때 발생하는 Propagation delay는 다음~\eqref{eq:propagation_delay}과 같은 식으로 계산할 수 있다.

\begin{align}
    \text{Propagation\;Delay} = \frac{\text{Distance\;between\;Tx\;-\;Rx}}{\text{Transmission\;Speed}}
    \label{eq:propagation_delay}
\end{align}
where Tx and Rx mean the transceiver and receiver, respectively. If the transmission speed is the same, it can be seen that the propagation delay is proportional to the distance between the two terminals according to~\eqref{eq:propagation_delay}. Fig.~\ref{fig:Propagation_delay} shows that the one-way propagation delay is as long as 1--2 ms when the terrestrial UE transmits a packet for handover to the LEO satellite.
% 여기에서 Tx는 Transceiver, Rx는 Receiver를 의미하며, Transmission speed가 동일하다면 Propagation delay는 두 단말 간의 거리와 비례관계에 있다는 것을 식을 통해 알 수 있다. 이러한 식을 이용해 Transmission speed가 동일할 때 거리에 따른 Propagation delay를 계산한 Fig.~\ref{fig:Propagation_delay}를 통해서, 지상의 UE가 저궤도 위성 네트워크에게 핸드오버를 위한 패킷을 전달할 때 one-way propagation delay가 1--2ms 정도로 길다는 것을 알 수 있다.

\begin{table}[]
  \centering
  \resizebox{1\linewidth}{!}{\begin{minipage}[t]{0.5\textwidth}
  \caption{Satellite parameters of \textbf{LEO-600}\\for system level simulator calibration~\cite{network2019atis}.}
  \centering
  \input{Table/Table_NTNparameter_3GPP.tex}
  \scriptsize
  \centering
  \label{tab:LEO-600}
  \end{minipage}}
\end{table} 

\begin{table}[]
%\small
    \caption{Parameters of $\mathrm{K_u}$-band terminal in~\eqref{eq:SNR}--\eqref{eq:FSPL}.}
    \label{tab:terminal_parameter}
    \centering
    \begin{tabular}{c||l}
        \toprule[1.0pt]
        Parameter & Value\\
        \midrule[1.0pt]
        BUC Operating Power & 16\,W (12\,dBW)\\
        Atmospheric Loss & 0.35\,dB\\
        Boltzmann Constant, $k$ & -228.6\,dBW/K/Hz\\
        Signal Frequency, $f$ & 14.25\,GHz\\
        Speed of Light in a Vacuum, $c$ & 3\,$\times$\,$10^8$\,m/s\\
        \bottomrule[1.0pt] 
    \end{tabular}
\end{table}

Next, immense uplink signal power is required to use the existing handover method in an LEO satellite network due to the physical distance. Table.~\ref{tab:LEO-600} shows satellite parameters for LEO-600 in orbit at an altitude of 600\,km. By calculating the signal-to-noise ratio (SNR), it is possible to estimate the uplink transmit power required when the UE periodically transmits packets to the LEO satellite in the uplink to check the handover condition. SNR refers to the ratio of how much noise is mixed in a receiver's signal compared to a transmitter's signal. Therefore, we can estimate the transmit power that sends a packet to the receiver with a decent signal by calculating SNR. This paper considers the Ka-band with channel bandwidth in the range of 25.5--40\,GHz used for radar and satellite communication to calculate the SNR for uplink in communication between LEO-600 and UE. In the following equation, we can calculate the SNR in an actual situation where a fixed u7 Ku-band terminal located in Seattle sends an uplink signal to LEO-600 in a broadside orientation.
% 다음으로, 기존 핸드오버 방식을 저궤도 위성 네트워크에서 사용하기 위해서는 물리적인 거리로 인한 큰 uplink signal power가 필요하다는 문제가 있다. Table.~\ref{tab:LEO-600}는 고도 600km의 궤도에 존재하는 \textit{LEO-600}에 대한 satellite parameters를 보여준다. Signal-to-Noise Ratio (SNR)을 계산함으로써, 핸드오버 조건을 검사하기 위해서 UE가 주기적으로 Satellite에게 uplink에 해당하는 Return (RTN) Link를 통해 패킷을 전달할 때 필요한 uplink transmit power를 추정할 수 있다. SNR이란, 송신단에서 보낸 신호에 비해 수신단에서 수신된 신호에 잡음이 얼마나 섞여 있는가를 비율을 의미한다. 따라서 SNR을 계산하면 어느 정도의 transmit power로 packet을 전송해야 수신단에 적절한 신호로 도달할지 추정할 수 있다. 본 논문에서는 실제 LEO-600과 UE와의 통신에서 uplink에 대한 SNR을 계산하기 위해 주로 radar와 limited number of satellite communication을 위해 사용하는 25.5--40\,GHz 범위의 channel bandwidth를 갖는 Ka--band를 고려한다. Seattle에 위치한 고정된 \textit{u7 Ku-band terminal}이 broadside orientation $(\theta=0)$인 상황에서 \textit{LEO-600}을 향해 uplink signal을 보내는 실제 상황에서의 \textsf{SNR}을 아래의 계산식을 통해 구할 수 있다.

\begin{align}
\begin{split}
    \textsf{SNR}\;(dB) = \textsf{BUC\;Operating\;Power}\;(dBW) +\; \textsf{G}\;(dBi) \\
    -\;\textsf{Atmospheric\;Loss}\;(dB) +\;\textsf{G/T\;of\;Satellite}\;(dB/K) \\
    -\;\textsf{k}\;(dBW/K/Hz) -\;\textsf{FSPL}\;(dB)
    \label{eq:SNR}
\end{split}
\end{align}
\textsf{BUC Operating Power} stands for the operating power of the block-up converter (BUC) that converts the frequency band from low frequency to high frequency for satellite signal transmission, and \textsf{G} is the maximum antenna gain of LEO-600. Next, \textsf{Atmospheric Loss} is the loss due to the attenuation of the electromagnetic wave signal in the air, and \textsf{G/T of Satellite} is an index representing the performance of the antenna according to the temperature expressed as the ratio of the antenna gain to the equivalent noise temperature of the receiver. Finally, \textsf{k} represents the theoretical noise floor or the minimum sensitivity of the receiver as the Boltzmann constant, and free space path loss (\textsf{FSPL}) is the path loss of the electromagnetic wave signal when communicating in free space calculated by~\eqref{eq:FSPL}.
% \textsf{BUC Operating Power}는 위성 신호 전송을 위해 주파수 대역을 낮은 주파수에서 높은 주파수로 변환하는 Block up converter (BUC)의 operating power에 해당하며, \textsf{G}는 \textit{LEO-600}의 안테나 gain에 해당하는 Satellite Rx max Gain이다. 다음으로 \textsf{Atmospheric Loss}는 대기에서 전자기파 신호의 감쇠로 인한 loss이고, \textsf{G/T of Satellite}은 안테나이득 (G)와 수신기의 등가 잡읍 온도 (T)의 비율로 표현되는 온도에 따른 안테나의 성능을 나타내는 지수이며, \textsf{k}는 Boltzmann Constant로 theoretical noise floor나 receiver의 minimum sensitivity를 나타낸다. 마지막으로 free space path loss (\textsf{FSPL})는 자유공간에서 통신할 때의 전자기파 신호의 path loss로, 아래의 식을 통해 계산할 수 있다.

\begin{equation}
    \textsf{FSPL}\;(dB) = 20\log_{10}(d) + 20\log_{10}(f) - 20\log_{10}(\frac{4\pi}{c})
    \label{eq:FSPL}
\end{equation}
where $d$, $f$, and $c$ are the distance between the UE and satellite, signal frequency of the UE, and speed of light in a vacuum, respectively. In~\eqref{eq:SNR}--\eqref{eq:FSPL}, the parameter values for the UE are summarized in Table.~\ref{tab:terminal_parameter}. Through this calculation process, the UE generally has an SNR of about 14.55--17.47\,$dB$ when transmitting a packet for handover to the LEO satellite network.

Regarding communication theory, the bit error ratio (BER) can evaluate link budget and outage probability for a given SNR. BER means the number of bits with errors in the transmit process relative to the number of received bits. In general, the relationship between SNR and BER is inversely proportional. This paper calculates BER through the following equation based on 64-quadrature amplitude modulation (QAM), which has 64 constellation sizes to process 6-bit data simultaneously used in satellite communication~\cite{BER_Calculation}.
% \eqref{eq:SNR}--\eqref{eq:FSPL}식에서 UE에 대한 parameter의 값은 Table.~\ref{tab:terminal_parameter}에 정리하였다. 이러한 계산 과정을 통해, 일반적으로 UE가 저궤도 위성 네트워크에게 핸드오버를 위한 패킷을 전달할 때 약 14.55--17.47\,$dB$의 \textsf{SNR}을 갖는다는 것을 알 수 있다.
% 통신 이론 측면에서 주어진 \textsf{SNR}에 대해서 Link budget과 outage probability를 평가할 때 bit error ratio (BER)을 들어 설명할 수 있다. BER이란 수신된 비트의 수에 대해 전달되는 과정에서 오류가 발생한 비트의 수를 의미하며, 일반적으로 \textsf{SNR}과 \textsf{BER}의 관계는 반비례이다. 본 논문에서는 실제 Satellite 통신에서 사용하는 Quadrature Amplitude Modulation (QAM) 중, 6-bit의 데이터를 한 번에 처리할 수 있는 64개의 constellation size의 64-QAM을 기반으로 아래의 식을 통해 \textsf{BER}을 계산한다~\cite{BER_Calculation}.
\begin{equation}
    \textsf{BER} = \frac{4}{k}\left(1-\frac{1}{\sqrt{M}}\right)\cdot\frac{1}{2}\mathrm{erfc}\left(\sqrt{\frac{3k\cdot10^{\frac{\textsf{SNR}}{10}}}{2(M-1)}}\right)
\end{equation}
subject to
\begin{equation}
    \mathrm{erfc}(z)=1-\mathrm{erf}(z)=1-\frac{2}{\sqrt{\pi}}\int_{0}^{z}e^{-t^2}dt
\end{equation}
where $k=\log_2(M)=6$ and $M=64$ stand for the bits per symbol and constellation size in 64-QAM, respectively. As illustrated in Fig.~\ref{fig:BER}, we can see that the BER has values from $1.3\times10^{-3}$ to $1.89\times10^{-5}$ in ground UE to LEO satellite communication. Therefore, it is necessary to further reduce BER in ground UE to LEO satellite communication link, which imposes a power consumption burden on the ground UE due to a higher power level. This paper proposes a novel DRL-based handover algorithm to solve the abovementioned problems to eliminate the burden of such ground UE's uplink signaling power and propagation delay.

% As shown in Fig.~\ref{fig:BER}, 식~\eqref{eq:SNR}을 통해 계산한 uplink in ground UE to LEO satellite에서 갖는 약 14.55--17.47\,$dB$의 \textsf{SNR}에 의해 from $1.3\times10^{-3}$ to $1.89\times10^{-5}$의 \textsf{BER}이 나타나는 것을 알 수 있다. 따라서, 일반적으로 ground UE to LEO satellite 통신에서는 \textsf{BER}을 더 줄일 필요가 있으며, 이는 더 높은 수준의 power가 요구되기 때문에 ground UE에게 파워 소모적인 부담을 준다. 따라서, 본 논문에서는 그러한 ground UE의 uplink signalling power에 대한 부담을 없애기 위해 novel한 핸드오버 알고리즘을 제안한다.


% \subsection{Challenge: High Spatial Correlation among Ground UEs}

%%% Illustrative Example


\subsection{Proposed Scheme}
% 제안 기법
As mentioned above, there are numerous limitations in applying the existing handover method equally to the LEO satellite network. Since the physical distance between the ground UE and the LEO satellite is far, a long propagation delay is consumed when handover packets are transmitted using the existing handover method. Accordingly, it is not easy to check the handover condition by reflecting the real-time information of the UE. In addition, it is inefficient in terms of power cost consumption because enormous uplink signaling power is consumed when handover packets are transmitted. Moreover, the \texttt{MR} containing network information to which the UE is connected must be periodically transmitted to the S-gNB so that it can check the handover status, as shown in Fig.~\ref{fig:existing scheme}. Therefore, several packet transfers occur by checking the handover entry condition between several UEs and the gNB. Efficiently adjusting propagation delay and uplink signaling power is consequential in performing a handover process in an LEO satellite network. As depicted in Fig.~\ref{fig:proposed scheme1}, this paper proposes a solution to the existing handover method's limitations due to the UE terminal's communication capability and the physical distance from the LEO satellite in the handover preparation phase. In this paper, we propose a method in which the S-gNB agent predicts the UE's network signal information using the period pattern of the LEO satellite networks based on deep reinforcement learning and delivers the \texttt{HO Request} to the T-gNB without \texttt{MR}. This scheme can solve the limitations of existing handover methods in LEO satellite networks since the S-gNB agent saves access delay time and power consumption in uplink signals for handover processing. The T-gNB performs handover based on the \texttt{HO Request} received from the S-gNB. In summary, the handover method proposed in this paper simplifies the preparation phase by predicting when the S-gNB agent should perform the handover based on deep reinforcement learning. The access delay for handover can be decreased by reducing the propagation delay via the proposed method. We can also save the signaling power for packet forwarding, while the handover performance can also be improved.
% 위에서 언급했듯이, 기존 핸드오버 방식을 저궤도 위성 네트워크에서 동일하게 적용하는 것은 많은 한계가 있다. 지상의 UE와 저궤도 위성 네트워크의 물리적인 거리가 많이 떨어져있기 때문에 기존 핸드오버 방식을 사용하여 핸드오버를 위한 패킷을 전달하게 되면, 매우 긴 propagation delay가 소모되기 때문에 UE의 실시간 정보를 반영하여 핸드오버 조건을 검사하기 어렵다. 또한, 핸드오버 수행을 위한 패킷을 전달할 때 큰 uplink signalling 파워가 소모되기 때문에 power의 cost 소모 관점에서도 효율적이지 않다. Moreover, Fig.~\ref{fig:existing scheme}에서 알 수 있듯이, UE의 핸드오버 조건을 검사하기 위해서는 주기적으로 UE가 연결되어 있는 네트워크 정보가 담긴 \texttt{Measurement Report}를 S-gNB에게 전송하여 해당 S-gNB가 핸드오버 수행 조건을 검사해야 한다. 따라서 여러 개의 UE들과 gNB 간에 \texttt{Measurement Report}를 통해 핸드오버 진입 조건을 검사하는 것 만으로도, 여러 번의 패킷 전달이 발생하기 때문에 propagation delay 및 uplink signalling power를 효율적으로 조절하는 것은 저궤도 위성 네트워크에서 핸드오버 과정을 수행하는 데에 있어 매우 중요하다. 따라서 본 논문에서는 Fig.~\ref{fig:proposed scheme1}와 같이 Handover preparation phase에서 UE 단말의 통신능력과 저궤도 위성 네트워크와의 물리적 거리로 인한 기존 핸드오버 방식의 한계를 해결한다. 본 논문에서는 저궤도 위성 네트워크에서 효과적으로 핸드오버를 수행하도록 하기 위해서 핸드오버 진입 조건을 검사하는 \texttt{Measurement Report} 없이 S-gNB 에이전트가 심층 강화학습을 기반으로 저궤도 위성들의 pattern 주기 정보를 이용해 UE의 네트워크 신호 정보를 예측하여 T-gNB에게 HO Request를 전달하는 방식을 제안한다. 이를 통해 핸드오버의 처리를 위한 Access delay 시간을 단축시킬 수 있으며, uplink signal에 소모되는 power도 save 할 수 있기 때문에 기존 핸드오버 방식이 저궤도 위성 네트워크에서 가지는 한계를 해결할 수 있다. T-gNB는 S-gNB에게 전달 받은 \texttt{HO Request}를 기반으로 핸드오버를 수행하게 된다. 정리하자면, 본 논문에서 제안하는 핸드오버 방식은 기존의 핸드오버 방식을 저궤도 위성 네트워크에서 그대로 사용할 때 발생하는 물리적인 한계를 극복하기 위해서 심층강화학습을 기반으로 하여 S-gNB 에이전트가 핸드오버를 수행해야 하는 시기를 예측함으로써, 핸드오버 과정 중 preparation phase에서 몇가지 단계를 생략하여 간략화한다. 이를 통해 핸드오버 과정 중의 propagation delay를 줄여 핸드오버를 위한 access delay를 감소시키고, 패킷 전달을 위한 signalling power를 save 하는 동시에 핸드오버의 성능 또한 향상시킬 수 있는 novel handover process를 제안한다.

\begin{figure*}[t!]
    \centering
    \subfloat[Existing 3GPP 5G handover preparation phase.]{
    \includegraphics[width=0.8\columnwidth]{Figure/Fig_HO_NTN_Baseline.png}
    \label{fig:existing scheme}
    }
    \subfloat[Proposed DRL-based handover preparation phase.]{
    \includegraphics[width=0.8\columnwidth]{Figure/Fig_HO_NTN_Proposed.png}
    \label{fig:proposed scheme1}
    }
    \\
    \caption{The sequence diagrams of existing and proposed 3GPP 5G handover preparation schemes.}
    \label{fig:preparation schemes}
\end{figure*}


==> Section/Repo/SEC4_CY.tex <==
\subsection{\tred{Algorithm Details}}
For DHO, the importance-weighted actor learner architecture (IMPALA) is used to train DRL agents~\cite{espeholt2018impala}. IMPALA is an off-policy reinforcement learning algorithm that learns through parallel actor-runners identical to the A3C algorithm~\cite{mnih2016asynchronous} of the same distributed RL method. In off-policy training, the learning process becomes unstable due to the significant variance caused by the policy lag between two different policies. In order to resolve policy lag, IMPALA uses a \emph{V-trace target}, which determines values through truncated importance sampling. Compared to the A3C algorithm, IMPALA is superior in learning speed and performance. Moreover, it has more stable characteristics in terms of hyperparameters and model structure.
 % 본 논문에서는 DRL의 에이전트들을 학습하기 위해서 Importance Weighted Actor Learner Architecture (IMPALA)~\cite{espeholt2018impala} 학습 알고리즘을 사용하였다. IMPALA는 같은 DistribUEed RL 방식의 A3C 알고리즘~\cite{mnih2016asynchronous}과 동일하게 parallel한 actor-runner를 통해 학습을 진행하는 off-policy 방식의 강화학습 알고리즘이다. Off-policy 방식의 training에서는 서로 다른 두가지의 Policy 간의 차이 (policy-Lag)로 인해 Variance가 크기 때문에 학습이 불안정해지지만, IMPALA에서는 Policy-Lag 문제를 해소하기 위해 Truncated Importance Sampling을 통해 Value를 결정하는 V-Trace Target을 사용한다. IMPALA는 A3C 알고리즘에 비해 학습 속도와 성능 면에서 보다 뛰어나며, 하이퍼파라미터 및 모델 구조의 측면에서 보다 안정적인 특징을 가지고 있다. 
IMPALA updates the policy by directly delivering the experiences collected by parallel actors making decisions in the environment to the global network. IMPALA updates the policy by directly delivering the experiences collected by parallel actors making decisions in the environment to the global network. Unlike A3C, where actors deliver gradients calculated using their collective experiences to the global network, IMPALA's global network is different in that it updates its policy through batches formed using experiences collected by actors. At this time, the V-trace method helps the learner to use the experience collected from different actors. The process for learners to update their policies in IMPALA is as follows:
% IMPALA는 parallel한 Actor들이 환경에서 의사 결정을 내리면서 수집한 Experience들을 Global Network에게 바로 전달하여 Policy를 업데이트한다. Actor가 자신이 수집한 Experience를 사용해 계산한 Gradient를 Global Network에게 전달하는 A3C와 다르게, IMPALA의 Global Network는 Actor들이 수집한 Experiement를 사용해 구성한 batch를 통해 자신의 policy를 업데이트한다는 점에서 차이가 있다. 이 때 V-Trace 방법을 사용하여 서로 다른 Actor로부터 수집된 Trajectory를 Learner가 그대로 사용할 수 있도록 해준다. IMPALA에서 Learner가 자신의 Policy를 Update하는 과정은 다음과 같다.
\begin{enumerate}
    \item Initialize and update the actor's policy based on the current learner's policy. % 현재 Learner의 Policy를 기반으로 Actor의 Policy를 업데이트한다.
    \item The actor collects experience in environments. % 일정 시간 동안 Actor의 Experience를 수집한다.
    \item The actor delivers the collected experience and its policy to the learner. % Actor가 수집한 Experience와 자신의 Policy를 Learner에게 전달한다.
    \item Learner trains its policy based on the experience and policy it receives. % Learner는 전달받은 Experience와 Policy를 바탕으로 자신의 Policy를 학습한다.
\end{enumerate}
Since IMPALA is an asynchronous distributed training model, even if different actors update their policies based on the same learner, they may differ due to differences in viewpoints. The detailed sequential process of the training algorithm is described in Algorithm~\ref{alg:IMPALA}.
% IMPALA는 Asynchronous DistribUEed Training Model이기 때문에 서로 다른 Actor가 같은 Learner를 기반으로 자신의 Policy를 업데이트하더라도 시점 차이에 의해 서로 다를 수 있다.


\subsubsection{V-Trace Target}
V-Trace conducts importance sampling (IS) when evaluating the value of experience because it uses experiences collected by different policies. The importance sampling ratio, which is the probability that the experience collected in the behavior policy appears in the target policy, is defined as follows:
% V-Trace란, 서로 다른 Policy에 의해 수집된 Trajectory를 사용하는 만큼, Experience에 대한 Value를 평가할 때에 Importance Sampling (IS)을 해주자는 것이다. Behavior Policy $\mu$에서 수집한 Trajectory가 Target Policy $\pi$에서도 나타날 확률인 Importance Sampling Ratio를 다음과 같이 정의한다.
\begin{equation}
\begin{split}
    & \rho_{t:T-1} \\
    & = \frac{\prod_{k=t}^{T-1}\pi
    (A_k|S_k)p(S_{k+1}|S_k,A_k)}{\prod_{k=t}^{T-1}\mu
    (A_k|S_k)p(S_{k+1}|S_k,A_k)} \\
    & = \prod_{k=t}^{T-1} \frac{\pi(A_k|S_k)}{\mu(A_k|S_k)}
\end{split}
\end{equation}
IS is to use samples from other distribUEions in order of importance to obtain the expected value of a specific distribution. When applied to off-policy reinforcement learning, IS can be used for learning by assigning weights according to the probability of appearing in $\pi$, which is the target of experience update sampled along $\mu$. V-trace target $v$ in a specific state $s_t$ is defined as follows:
% 어떤 한 분포의 기대값을 구하기 위해 다른 분포에서 샘플링한 샘플들을 중요도(Importance)에 따라 사용하자는 것인데, 강화학습의 Off-Policy 개념에 적용해보면 $\mu$ 를 따라 샘플링한 Experience 업데이트의 대상이 되는 $\pi$에서 나타날 확률에 따라 가중치를 부여하여 학습에 사용할 수 있다. 어떤 State $s_t$에서의 V-Trace Target $v$는 다음과 같이 정의된다.
\begin{equation}
    v_{s_t}\overset{\underset{\mathrm{def}}{}}{=} V(s_t)+\sum_{k=t}^{t+n-1}\gamma^{k-t}(\prod_{i=t}^{k-1}c_i\delta_k V)
\end{equation}
where $\delta_k V \overset{\underset{\mathrm{def}}{}}{=} \rho_k(r_k+\gamma V(s_{k+1})-V(s_k))$ is a temporal difference for the value function. $c_i\overset{\underset{\mathrm{def}}{}}{=} \min \left(\bar{c}, \frac{\pi(a_i|s_i)}{\mu(a_i, s_i)}\right)$ and $\rho_k\overset{\underset{\mathrm{def}}{}}{=} \min\left(\bar{\rho}, \frac{\pi(a_k|s_k)}{\mu(a_k, s_k)}\right)$ $(\bar{\rho}\ge\bar{c})$ are the Truncation level of the IS weights. Lower bounds $\bar{c}$, $\bar{\rho}$ called truncated importance sampling weights are set so that the weights do not fall below a certain level. Here, $c$ is the cumulative weight accumulated up to the $k$-th step, and $\rho$ is the weight applied to the temporal difference $r_k+\gamma V(s_{k+1})-V(s_k)$ of the $k$-th step when obtaining the target in the $n$-step. In this respect, $\rho$ applied directly to the temporal difference value affects the convergence direction of the value function. The following is the convergence direction of the policy considering the different value functions.
% 이 때 일정 수준 이하로는 Weight가 떨어지지 않도록 Lower Bound를 설정하고 있는데, 이를 Truncated Importance Sampling Weight라고 한다. 여기서, $n$-step Target을 구할 때 $k-1$ step까지는 $c$가 적용되고 마지막 $k$번째 Step에서는 $\rho$가 적용됨을 알 수 있다. $\rho$는 $k$번째 Step의 Temporal Difference $r_k+\gamma V(s_{k+1})-V(s_k)$에 적용되는 Weight이고, $c$는 $k$번째 Step에 도달하는 과정에서의 누적되는 Weight이다. 이러한 점에서 Temporal Difference 값에 곧바로 적용되는 $\rho$는 Value Function의 수렴 방향(Fixed Point)에 영향을 미친다. 따라서, Value Function이 달라지기 때문에 Policy의 수렴 방향은 아래와 같다.
\begin{equation}
    \pi_{\bar{\rho}}\overset{\underset{\mathrm{def}}{}}{=}\frac{\min(\bar{\rho}\mu(a|s))}{\sum_{b\in A}\min(\bar{\rho}\mu(b|s),\pi(b|s))}
\end{equation}
If the value of $\bar{\rho}$ is infinite, the value of $\rho$ will always be $\frac{\pi(a|s)}{\mu(a|s)}$. In other words, the value function becomes the same as the target policy $\pi$ since truncation of IS weight is not applied. Conversely, it becomes closer than the behavior policy $\mu$ as the value of $\rho$ approaches zero. On the other hand, since $c$ is not directly applied to the temporal difference, it does not affect the update direction of the value function. It plays a role in adjusting the update speed according to how frequently the current experience occurs.
% 만약 $\bar{\rho}$의 값이 무한이라면, $\rho$의 값은 항상 $\frac{\pi(a|s)}{\mu(a|s)}$가 된다. 즉, Importance Sampling Weight에 대한 Truncation이 전혀 되지 않는다는 것이기 때문에 Value Function은 Target Policy $\pi$와 동일해진다. 반대로 $\rho$의 값이 0에 가까워질수록 Behavior Policy $\mu$보다 가까워게 된다. 반면 $c$는 Temporal Difference에 곧장 적용되는 것이 아니므로 Value Function의 업데이트 방향에는 영향을 미치지 않는다. 다만 현재 사용하고 있는 Trajectory가 얼마나 빈번하게 발생하는지에 따라 업데이트 속도를 조절하는 역할을 한다고 볼 수 있다.

\subsubsection{Update Direction by Policy Gradient}
This subsection will describe the process of training the agent's policy. The following is the actor-critic policy gradient considering the action-value function. % Action-value function을 통해 고려한 Actor-Critic의 Policy Gradient는 다음 식과 같다.
\begin{equation}
    \nabla_\theta J(\theta) = \mathbb{E}_\tau\big[\sum_{t=0}^{T-1}\nabla_\theta\log\pi_\theta(a_t|s_t)Q(s_t, a_t)\big]
\end{equation}
Suppose $\mu$ and $\pi$ are different from each other as an off-policy rather than an on-policy. In that case, the direction of policy update in state $s_t$ can be determined by multiplying the importance sampling ratio as follows:
% On-Policy가 아닌 Off-Policy로서 $\mu$와 $\pi$가 서로 다르다면, Importance Sampling Ratio를 곱해주어 다음과 같이 한 State $s_t$에서의 Policy의 업데이트 방향을 결정할 수 있다.
\begin{equation}
    \mathbb{E}_{a_s\sim\mu(\cdot|s_t)}\big[
    \frac{\pi_{\bar{\rho}}(a_t|s_t)}{\mu(a_s|x_s)}
    \nabla\log\pi_{\bar{\rho}}(a_t|s_t)q_t|s_t\big]
\end{equation}
where $q_t\overset{\underset{\mathrm{def}}{}}{=}r_t+\gamma v_{t+1}$ is an estimate of $Q^{\pi_{\bar{\rho}}}(s_t,a_t)$.

\subsubsection{V-Trace Actor-Critic Algorithm}
The update loss calculated by IMPALA consists of the following three things; (i) Policy Gradient Loss, (ii) Baseline Loss, and (iii) Entropy Loss. First, IMPALA reduces the distance from the V-trace target $v$ when updating the baseline $V(s)$ as follows:
% IMPALA에서 구할 Update Loss는 다음 세 가지로 구성된다; (i) Policy Gradient Loss, (ii) Baseline Loss, and (iii) Entropy Loss. 먼저, Baseline $V(s)$를 업데이트 할 때에는 V-Trace Target $v$와의 거리를 다음 식과 같이 줄이도록 한다.
\begin{equation}
    (v_t - V_\theta(s_t))\nabla_\theta V_\theta(s_t)
\end{equation}
Next, a temporal difference term can be constructed using the advantage $r_t+\gamma v_{t+1}-V_w(s_t)$ obtained by subtracting the baseline from the action value function $Q(s,a)$ in the following equation.
% 다음으로, Action value function $Q(s,a)$에서 Baseline $V(s)$를 뺀 Advantage $r_t+\gamma v_{t+1}-V_w(s_t)$를 사용하여 다음 식과 같이 Temporal Difference Term을 구성할 수 있다.
\begin{equation}
    \rho_t \nabla_\omega \log\pi_\omega(a_t|s_t)(r_t+\gamma v_{t+1}-V_\theta(s_t))
\end{equation}
In this way, using the advantage of subtracting the baseline for the action value function reduces the variance of the policy gradient. Note that $V$ is the value function, and $v$ is the V-Trace Target. Finally, entropy loss is introduced to ensure sufficient exploration and prevent premature convergence like A3C.
% 이처럼 Action Value Function에 Baseline을 빼준 Advantage를 사용하게 되면 Policy Gradient의 Variance가 줄어든다는 장점을 가진다. 마지막으로 A3C에서 도입하였듯이 충분한 Exploration이 이뤄지도록 하고, premature convergence를 막기 위해 Entropy Loss를 도입하고 있다.
\begin{equation}
    -\nabla_\omega \sum_a\pi_\omega(a|s_t)\log\pi_\omega(a|s_t)
\end{equation}

\begin{algorithm}[t]
    Initialize the \textit{learner} network's weights $\phi$ $\rightarrow$ $\phi_0$\,;\\
    \For{Epoch = 1, MaxEpoch}{
        \For{each \textit{actor} $i$, $\forall i \in [1,I]$}{
        $\triangleright$ \textbf{Initialize LEO Satellite Environments} :\,\,
        Set replay buffer $\mathcal{D}_i=\{\}$ and $s$ $\rightarrow$ $s_0\,;$ \\

        $\triangleright$ Update \textit{actor} weight $\theta_i$ from the \textit{learner} : Download weights $\theta_i$ = $\phi\,;$ \\
        
        \While{$t < \text{episode limit}$}{    
            $\triangleright$ Select the action $a^t_i$ based on its policy $\mu_{\theta_i}(a_i^t\,|\,s_i^t)$ at time step $t\,;$ \\
            $\triangleright$ Get reward $r_i^t$ and move $s_i^t \rightarrow s^{t+1}\,;$ \\
            $\triangleright$ Set experience $\xi^t_i= \{s_i^t, a_i^t, r_i^t, s_i^{t+1}\}\,;$ \\
            $\triangleright$ Update replay buffer : $\mathcal{D}_i=\mathcal{D}_i\cup\xi^t_i\,;$ \\
            }
        $\triangleright$ Upload $\mu_{\theta_i}$ and $\mathcal{D}_i$ to the \textit{learner}$\,;$ \\
        $\triangleright$ Update weights $\phi$ of the \textit{learner} network $\pi_\phi$ on the basis of the $\mu_{\theta_i}$ and $\mathcal{D}_i\,;$
        }
    }
    \caption{Training algorithm of IMPALA for the proposed 3GPP 5G HO scheme (???)}
    \label{alg:IMPALA}
\end{algorithm}
